Minimal regret state estimation of time-varying systems

Kalman and H-infinity filters, the most popular paradigms for linear state estimation, are designed for very specific specific noise and disturbance patterns, which may not appear in practice. State observers based on the minimization of regret measures are a promising alternative, as they aim to adapt to recognizable patterns in the estimation error. In this paper, we show that the regret minimization problem for finite horizon estimation can be cast into a simple convex optimization problem. For this purpose, we first rewrite linear time-varying system dynamics using a novel system level synthesis parametrization for state estimation, capable of handling both disturbance and measurement noise. We then provide a tractable formulation for the minimization of regret based on semi-definite programming. Both contributions make the minimal regret observer design easily implementable in practice. Finally, numerical experiments show that the computed observer can significantly outperform both H-2 and H-infinity filters.

==> noise_robust.tex <==
\pgfplotsset{
compat=1.11,
legend image code/.code={
\draw[mark repeat=2,mark phase=2]
plot coordinates {
(0cm,0cm)
(0.15cm,0cm)        %% default is (0.3cm,0cm)
(0.3cm,0cm)         %% default is (0.6cm,0cm)
};%
}
}


% This file was created with tikzplotlib v0.9.15.
\begin{tikzpicture}

\begin{axis}[
legend cell align={left},
legend columns=2,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(1,0.14), font=\small}, anchor=east, draw=white!80!black},
log basis x={10},
log basis y={10},
tick align=outside,
width=8cm,
height=5cm,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmajorgrids,
xmin=1e-05, xmax=0.001,
xmode=log,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ymin=0.01, ymax=1.22304407455456,
xtick={0.00001,0.00002,0.00005,0.0001,0.0002,0.0005,0.001},
xticklabels={$10^{-5}$,$2\cdot 10^{-5}$, $5\cdot 10^{-5}$, $10^{-4}$, $2\cdot 10^{-4}$, $5\cdot 10^{-4}$, $10^{-3}$},
ymode=log,
ytick style={color=black},
ytick={0.01,0.02,0.05,0.1,0.2,0.5,1},
yticklabels={1\%,2\%,5\%,10\%,20\%,50\%,100\%},
xlabel={noise level [p.u.]},
ylabel={relative estimation error}]
]
\path [draw=black, fill=black, opacity=0.2]
(axis cs:1e-05,0.0489842193570679)
--(axis cs:1e-05,0.0474157806429321)
--(axis cs:2e-05,0.150257670780787)
--(axis cs:5e-05,0.471762255228189)
--(axis cs:0.0001,0.72848141447824)
--(axis cs:0.0002,0.884079015518638)
--(axis cs:0.0005,0.969093798079768)
--(axis cs:0.001,0.989841886116992)
--(axis cs:0.001,0.990158113883008)
--(axis cs:0.001,0.990158113883008)
--(axis cs:0.0005,0.969906201920232)
--(axis cs:0.0002,0.886720984481362)
--(axis cs:0.0001,0.734418585521759)
--(axis cs:5e-05,0.481337744771811)
--(axis cs:2e-05,0.156442329219213)
--(axis cs:1e-05,0.0489842193570679)
--cycle;

\path [draw=blue, fill=blue, opacity=0.2]
(axis cs:1e-05,0.0181138357147217)
--(axis cs:1e-05,0.0144861642852783)
--(axis cs:2e-05,0.0178133931252681)
--(axis cs:5e-05,0.0324907630408086)
--(axis cs:0.0001,0.0604252717712433)
--(axis cs:0.0002,0.119290537823628)
--(axis cs:0.0005,0.312522590272842)
--(axis cs:0.001,0.781395318220831)
--(axis cs:0.001,0.935454681779169)
--(axis cs:0.001,0.935454681779169)
--(axis cs:0.0005,0.331977409727158)
--(axis cs:0.0002,0.123659462176372)
--(axis cs:0.0001,0.0627247282287567)
--(axis cs:5e-05,0.0342592369591914)
--(axis cs:2e-05,0.0207866068747318)
--(axis cs:1e-05,0.0181138357147217)
--cycle;

\path [draw=red, fill=red, opacity=0.2]
(axis cs:1e-05,0.0585284677683639)
--(axis cs:1e-05,0.0558215322316361)
--(axis cs:2e-05,0.1560751000016)
--(axis cs:5e-05,0.469397341177589)
--(axis cs:0.0001,0.724730151519017)
--(axis cs:0.0002,0.881558992781175)
--(axis cs:0.0005,0.968255033785326)
--(axis cs:0.001,0.989496464289287)
--(axis cs:0.001,0.989853535710714)
--(axis cs:0.001,0.989853535710714)
--(axis cs:0.0005,0.968994966214674)
--(axis cs:0.0002,0.884191007218825)
--(axis cs:0.0001,0.730669848480983)
--(axis cs:5e-05,0.478802658822411)
--(axis cs:2e-05,0.1623248999984)
--(axis cs:1e-05,0.0585284677683639)
--cycle;

\path [draw=green!50.1960784313725!black, fill=green!50.1960784313725!black, opacity=0.2]
(axis cs:1e-05,0.0195454769981818)
--(axis cs:1e-05,0.0154045230018182)
--(axis cs:2e-05,0.0155048763060678)
--(axis cs:5e-05,0.0179358996070273)
--(axis cs:0.0001,0.0246114661349286)
--(axis cs:0.0002,0.0424619603388562)
--(axis cs:0.0005,0.154629095035332)
--(axis cs:0.001,0.493550858982598)
--(axis cs:0.001,0.660899141017402)
--(axis cs:0.001,0.660899141017402)
--(axis cs:0.0005,0.183470904964668)
--(axis cs:0.0002,0.0514380396611438)
--(axis cs:0.0001,0.0280885338650714)
--(axis cs:5e-05,0.0209641003929727)
--(axis cs:2e-05,0.0193451236939322)
--(axis cs:1e-05,0.0195454769981818)
--cycle;

\addplot [semithick, black]
table {%
1e-05 0.0482
2e-05 0.15335
5e-05 0.47655
0.0001 0.73145
0.0002 0.8854
0.0005 0.9695
0.001 0.99
};
\addlegendentry{OLS}
\addplot [semithick, blue]
table {%
1e-05 0.0163
2e-05 0.0193
5e-05 0.033375
0.0001 0.061575
0.0002 0.121475
0.0005 0.32225
0.001 0.858425
};
\addlegendentry{MLE}
\addplot [semithick, red]
table {%
1e-05 0.057175
2e-05 0.1592
5e-05 0.4741
0.0001 0.7277
0.0002 0.882875
0.0005 0.968625
0.001 0.989675
};
\addlegendentry{Lasso}
\addplot [semithick, green!50.1960784313725!black]
table {%
1e-05 0.017475
2e-05 0.017425
5e-05 0.01945
0.0001 0.02635
0.0002 0.04695
0.0005 0.16905
0.001 0.577225
};
\addlegendentry{MAP}
\end{axis}

\end{tikzpicture}


\pgfplotsset{
compat=1.11,
legend image code/.code={
\draw[mark repeat=2,mark phase=2]
plot coordinates {
(0cm,0cm)
(0.3cm,0cm)        %% default is (0.3cm,0cm)
(0.6cm,0cm)         %% default is (0.6cm,0cm)
};%
}
}

==> vanderpol_output.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}[scale=0.48]

\begin{axis}[%
width=6.028in,
height=2.754in,
at={(1.011in,0.642in)},
scale only axis,
xmin=1,
xmax=21,
ymin=-2.5,
ymax=2.5,
axis background/.style={fill=white},
title style={font=\bfseries},
xmajorgrids,
ymajorgrids,
xlabel = {\Huge$t$},
ylabel = {\Huge$x$},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	-0.517621982318193\\
2	0.150294183125384\\
3	1.05339135411462\\
4	1.85826116731073\\
5	2.10695857055918\\
6	2.02327955292038\\
7	1.83737400560527\\
8	1.60174578296288\\
9	1.31454745288221\\
10	0.952085740140477\\
11	0.465675402428001\\
12	-0.224564649188416\\
13	-1.14148128511023\\
14	-1.90528635913629\\
15	-2.1076546852137\\
16	-2.00888053608687\\
17	-1.81757197738253\\
18	-1.57766295289079\\
19	-1.28482973509436\\
20	-0.913458536440307\\
21	-0.411995657610654\\
};
\addlegendentry{Exact}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	-0.46670253636758\\
2	0.148783762584071\\
3	0.972294451354883\\
4	1.73565615586282\\
5	2.0242780185617\\
6	1.96366047881051\\
7	1.77089116917861\\
8	1.52421168745254\\
9	1.23271126354034\\
10	0.878002160474488\\
11	0.41824677855353\\
12	-0.216548151432164\\
13	-1.05327172386061\\
14	-1.78400578108294\\
15	-2.02893439694265\\
16	-1.94939495220559\\
17	-1.74998278459066\\
18	-1.49935605723304\\
19	-1.20311820073026\\
20	-0.840902597552911\\
21	-0.368312925365872\\
};
\addlegendentry{Regret}

\addplot [color=mycolor3]
  table[row sep=crcr]{%
1	-0.540961819528869\\
2	0.0386163143649112\\
3	0.808302843151402\\
4	1.56616637396672\\
5	1.94824696851849\\
6	1.98045632229337\\
7	1.82840395814314\\
8	1.58784190270735\\
9	1.29234666622143\\
10	0.938651135240359\\
11	0.494473028480274\\
12	-0.102073927186132\\
13	-0.885289020312617\\
14	-1.61997810536146\\
15	-1.96325950743798\\
16	-1.97224418605365\\
17	-1.80919943034866\\
18	-1.5628482637253\\
19	-1.26255976351595\\
20	-0.902321688217795\\
21	-0.447076294021525\\
};
\addlegendentry{Kalman}

\addplot [color=mycolor4]
  table[row sep=crcr]{%
1	-0.306614883337843\\
2	0.404808352153851\\
3	1.35636273192471\\
4	2.16896552682074\\
5	2.33514866710281\\
6	2.13212260320229\\
7	1.84197284595373\\
8	1.52807563368395\\
9	1.18356702132449\\
10	0.776944404090186\\
11	0.250964980524366\\
12	-0.483531059214185\\
13	-1.44811185899748\\
14	-2.21198619096357\\
15	-2.3252476288611\\
16	-2.10709781258053\\
17	-1.81390223619847\\
18	-1.49795031030022\\
19	-1.14935492985317\\
20	-0.734619462414949\\
21	-0.193537751722898\\
};
\addlegendentry{Hinf}

\end{axis}

\begin{axis}[%
width=7.778in,
height=5.833in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
